Towards Scaling Blockchain Systems via Sharding

Existing blockchain systems scale poorly because of their distributed consensus protocols. Current attempts at improving blockchain scalability are limited to cryptocurrency. Scaling blockchain systems under general workloads (i.e., non-cryptocurrency applications) remains an open question. In this work, we take a principled approach to apply sharding, which is a well-studied and proven technique to scale out databases, to blockchain systems in order to improve their transaction throughput at scale. This is challenging, however, due to the fundamental difference in failure models between databases and blockchain. To achieve our goal, we first enhance the performance of Byzantine consensus protocols, by doing so we improve individual shards' throughput. Next, we design an efficient shard formation protocol that leverages a trusted random beacon to securely assign nodes into shards. We rely on trusted hardware, namely Intel SGX, to achieve high performance for both consensus and shard formation protocol. Third, we design a general distributed transaction protocol that ensures safety and liveness even when transaction coordinators are malicious. Finally, we conduct an extensive evaluation of our design both on a local cluster and on Google Cloud Platform. The results show that our consensus and shard formation protocols outperform state-of-the-art solutions at scale. More importantly, our sharded blockchain reaches a high throughput that can handle Visa-level workloads, and is the largest ever reported in a realistic environment.

==> tables/OmniL_comsize.tex <==
\begin{table}[t]
\centering
\caption{Required committee size against $s\%$ attackers, to ensure failure probability below $2^{-20}$.}
\label{tab:omni_com_size}
\begin{tabular}{ccccccccc}
\hline
$s\%$ & & 0    & 5    & 10   & 15   & 20 & 25 & 30    \\
\hline
Committee size & & 1    & 28    & 55   & 106   & 227 & 648 & 4625    \\
\hline
\end{tabular}
\end{table}


==> tables/TCB_size.tex <==
\begin{table}[]
\centering
\caption{TCB size (LoC) of different trusted modules.}
\label{tab:tcb_size}
\begin{tabular}{ccccc}
\hline
\poet & \spoet    & AHL & \textproc{E-AggrSign}   & \textproc{E-RandGen}    \\
\hline
1300    & 1310    & 780   & 130   & 100\\
\hline
\end{tabular}
\end{table}


==> tables/bandwidth_heatmap.tex <==
\begin{table*}[t] \centering
\caption{Selected Bandwidth on Google Compute Engine (Mbits/s)}
\label{table:bw-gce}
\resizebox{0.9\textwidth}{!} {
\begin{tabular}{|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{Zone} & \textbf{us-west1-b} & \textbf{us-west2-a} & \textbf{us-east1-b} & \textbf{us-east4-b} & \textbf{asia-east1-b} & \textbf{asia-southeast1-b} & \textbf{europe-west1-b} & \textbf{europe-west2-a} \\
\hline\hline
\textbf{us-west1-b} & 0.0 & \cellcolor{grad_1} 36.6 & \cellcolor{grad_0} 13.6 & \cellcolor{grad_0} 15.6 & \cellcolor{grad_0} 7.7 & \cellcolor{grad_0} 6.1 & \cellcolor{grad_0} 6.6 & \cellcolor{grad_0} 6.8 \\
\hline
\textbf{us-west2-a} & \cellcolor{grad_1} 36.6 & 0.0 & \cellcolor{grad_0} 14.4 & \cellcolor{grad_0} 15.1 & \cellcolor{grad_0} 7.2 & \cellcolor{grad_0} 5.7 & \cellcolor{grad_0} 6.5 & \cellcolor{grad_0} 6.8 \\
\hline
\textbf{us-east1-b} & \cellcolor{grad_0} 13.6 & \cellcolor{grad_0} 14.5 & 0.0 & \cellcolor{grad_2} 72.0 & \cellcolor{grad_0} 5.0 & \cellcolor{grad_0} 4.3 & \cellcolor{grad_0} 9.8 & \cellcolor{grad_0} 10.4 \\
\hline
\textbf{us-east4-b} & \cellcolor{grad_0} 15.5 & \cellcolor{grad_0} 15.1 & \cellcolor{grad_2} 70.7 & 0.0 & \cellcolor{grad_0} 5.3 & \cellcolor{grad_0} 4.4 & \cellcolor{grad_0} 11.2 & \cellcolor{grad_0} 12.0 \\
\hline
\textbf{asia-east1-b} & \cellcolor{grad_0} 7.7 & \cellcolor{grad_0} 7.2 & \cellcolor{grad_0} 5.0 & \cellcolor{grad_0} 5.3 & 0.0 & \cellcolor{grad_0} 18.2 & \cellcolor{grad_0} 5.9 & \cellcolor{grad_0} 3.7 \\
\hline
\textbf{asia-southeast1-b} & \cellcolor{grad_0} 6.1 & \cellcolor{grad_0} 5.7 & \cellcolor{grad_0} 4.3 & \cellcolor{grad_0} 4.4 & \cellcolor{grad_0} 18.1 & 0.0 & \cellcolor{grad_0} 3.2 & \cellcolor{grad_0} 3.3 \\
\hline
\textbf{europe-west1-b} & \cellcolor{grad_0} 10.5 & \cellcolor{grad_0} 6.5 &
\cellcolor{grad_0} 9.8 & \cellcolor{grad_0} 11.1 & \cellcolor{grad_0} 3.7 &
\cellcolor{grad_0} 3.2 & 0.0 & \cellcolor{grad_4} 127.0 \\
\hline
\textbf{europe-west2-a} & \cellcolor{grad_0} 6.9 & \cellcolor{grad_0} 6.9 & \cellcolor{grad_0} 10.4 & \cellcolor{grad_0} 11.9 & \cellcolor{grad_0} 3.8 & \cellcolor{grad_0} 5.2 & \cellcolor{grad_4} 126.0 & 0.0 \\
\hline
\end{tabular}
}
\end{table*}


==> tables/l_randfail.tex <==
\begin{table}[t]
\centering
\caption{Effect of $l$ on $P_{\tt RndFail}$ and expected communication complexity of \codename\ committee formation (\textit{Msg.} column). $n$ refers to the number of nodes, and $c$ is some constant.}
\label{tab:l_randfail}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{>{\raggedright\arraybackslash}m{3cm}>{\centering\arraybackslash}m{1cm}
>{\raggedleft\arraybackslash}m{2cm}}
\hline
$\textbf{l}$ & $\mathbf{2^{-l}}$ &  \textbf{Msg.} \\ \hline
$\log(n)$  & $1/n$ & $O(n)$ \\
$\log(n) - \log(\log(n))$ &   $\log(n)/n$ & $O(n \log(n))$ \\ 
$\log(n)/2$ &  $1/\sqrt{n}$ & $O(n \sqrt{n})$ \\ 
$\log(c)$ &  $1/c$ & $O(n^2)$ \\ \hline
\end{tabular}
}
\end{table}

==> tables/notation.tex <==
\begin{table}[t]
\centering
\caption{Summary of notations and abbreviations in this paper.}
\label{tab:notations}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|>{\color{blue}\centering\arraybackslash}m{2cm}||>{\color{blue}\arraybackslash}m{7cm}|}
\hline
 \textbf{Notation} 		&  \textbf{Description}                                  \\ \hline
 $n$      		&  {Number of nodes in the network}             \\ \hline
 $f$      		&  {Number of Byzantine failures}               \\ \hline
 $c$          & {Number of clients} \\ \hline
% $c_t$        & {number of threads per client} \\ \hline
 $r$      		&  {Request rate per client thread}                               \\ \hline
 $t$          & {View change time out} \\ \hline
 $k$      		&  Number of committees  				        \\ \hline
 $s$      		&  {Fraction of nodes under attacker's control}	\\ \hline
 \texttt{q}		& Random value determining node eligibility		\\ \hline
 $l$				& Bit-length of \texttt{q}						\\	\hline
 \hline
 HL & PBFT used Hyperledger Fabric v0.6\\ \hline
 AHL & PBFT-A2M~\cite{a2m} implemented for Hyperledger Fabric v0.6 \\ \hline
 AHL+ & AHL with request multicast removed and consensus messages prioritized (Section~\ref{subsec:scale_pbft}) \\ \hline
 AHLR & AHL with enclave-based collective signing \\ \hline
 \textproc{E-AggrSign} & The enclave implementing collective signing in AHLR \\ \hline
 AHLR+ & AHLR with request multicast removed and consensus messages prioritized \\ \hline
 \poet & Proof of Elapsed Time in Hyperledger Sawtooth v0.8 \\ \hline
 \spoet & \poet\ with effective network scaled down \\ \hline
 \codename & Our proposed sharding protocol with efficient committee formation and small committee size\\ \hline
  \textproc{E-RandGen} &  The enclave that implements trusted randomness beacon in \codename \\ \hline

 
\end{tabular}
}
\end{table}


==> tables/randhound_runtime.tex <==
\begin{table}[t]
\centering
\caption{\textcolor{blue}{RandHound runtime with group size $c=16$.}}
\label{tab:randhound_runtime}
\begin{tabular}{ccccccc}
\hline
n & & 32    & 64    & 128   & 256   & 512    \\
\hline
Time (s) & & 15.73 & 22.82 & 40.97 & 76.34 & 151.76 \\
\hline
\end{tabular}
\end{table}

==> tables/scaling_proposal_tab.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table*}
\centering
\caption{Summary of existing scaling protocols evaluated in this paper.}
\label{tab:scaling_summary}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{|>{\raggedright\arraybackslash}m{1.5cm}||>{\centering\arraybackslash}m{4.5cm}|>{\centering\arraybackslash}m{4.5cm}|>{\centering\arraybackslash}m{3.5cm}|>{\centering\arraybackslash}m{3.5cm}|}
%\begin{tabular}{c|c|c|c|}
\hline
& \textbf{AHL}~\cite{a2m}
& \textbf{AHLR}~\cite{a2m,byzcoin}
& \textbf{PoET}~\cite{poet}
& {\bf Elsatico \& Omniledger}\cite{elastico,omniledger}          \\ 
%\hline 
%Built Upon   &	PBFT~\cite{pbft_thesis} + A2M~\cite{a2m} & AHL + Byzcoin~\cite{byzcoin}  & Classical BFT + Nakamoto Protocols   & Nakamoto Protocol    \\ 
\hline
Network     & Permissioned & Permissioned  & Permissionless & Permissionless    \\ 
%\hline
%Trusted hardware & Yes & Yes & Yes  & No  \\ 
\hline
Design
& Employ trusted hardware to eliminate equivocation, requring only $n=2f+1$ nodes to tolerate $f$ Byzantine failures
& Aggregate messages at the leader, reducing communication complexity to $O(n)$
& Eliminate PoW by using Intel SGX as trusted random source 
& Divide nodes into multiple shards; each shard runs PBFT \\ 
\hline
%Consensus Finality      & Yes & Yes    & Yes  & No  \\ 
%\hline
\end{tabular}
}
\end{table*}

